Generalization of Graph-Based Active Learning Relaxation Strategies Across Materials

Although density functional theory (DFT) has aided in accelerating the discovery of new materials, such calculations are computationally expensive, especially for high-throughput efforts. This has prompted an explosion in exploration of machine learning assisted techniques to improve the computational efficiency of DFT. In this study, we present a comprehensive investigation of the broader application of Finetuna, an active learning framework to accelerate structural relaxation in DFT with prior information from Open Catalyst Project pretrained graph neural networks. We explore the challenges associated with out-of-domain systems: alcohol ($C_{>2}$) on metal surfaces as larger adsorbates, metal-oxides with spin polarization, and three-dimensional (3D) structures like zeolites and metal-organic-frameworks. By pre-training machine learning models on large datasets and fine-tuning the model along the simulation, we demonstrate the framework's ability to conduct relaxations with fewer DFT calculations. Depending on the similarity of the test systems to the training systems, a more conservative querying strategy is applied. Our best-performing Finetuna strategy reduces the number of DFT single-point calculations by 80% for alcohols and 3D structures, and 42% for oxide systems.

==> OOD_adsorbates_and_functional.tex <==
% Modeling alcohol dehydrogenation to aldehydes is a complex process full of nuances not yet considered in the \gls{oc20} dataset. In this experiment, we will explore these nuances and how they may or may not effect the performance of the FineTuna framework. 


% Here, we will be benchmarking the reaction energies ($E_{rxn}$) for a two-step dehydrogenation reaction which will require calculations of the alcohols as well as their radicals and final byproduct. By calculating the reaction energy and not just the adsorption energy, we will also demonstrate that FineTuna is able to shorten the relaxation trajectory for radicals of alcohols which is not something explored in the \gls{oc20} dataset. The first dehydrogenation step will be the dehydrogenation of the hydroxyl group followed by the second dehydrogenation step with the dehydrogenation of the C-H group bounded to the hydroxyl. 

% We explore $E_{rxn}$ for each molecule on three different surfaces of ternary materials with chemical compositions outside of the domain of \gls{oc20}. For each alcohol dehydrogenation reaction, we assessed $E_{rxn}$ for a ternary intermetallic, a binary intermetallic with a covalent anion, and a unary metallic system with two anions. The facet of these materials was randomly chosen from a set of facets with a max Miller index of 3 which are facets that are also out-of-domain from \gls{oc20}. 

% The purpose of this experiment is to:
% \begin{enumerate}
    % \item Assess the capability of FineTuna to predict trajectories for adsorbed slabs that are out of domain from the OC20 training set
    % \item Materials used to make the the slabs are out of domain in regards to the chemical composition. OC20 has never seen slabs made of these particular combination of elements before
    % \item To test chemical diversity of the slab systems, we assessed adsorption on three types of surfaces: ternary intermetallics (MMM), ternary bimetallics with an anion (MMX), and ternary unary metallic with two anions (MXX). 
    % \item We also want to assess the capabilities of FineTuna in regards to correctly determining the trajectory of out of domain adsorbates and their radicals.
    % \item We picked three alcohols for this experiment, a C3 2-propanol, C4 2-butanol, and C6 cyclohexanol. The training set of OC20 only assess carbon molecules up to C2, so these alcohols are out of doamin.
    % \item For each surface, we assess the reaction energy for a two-step dehydrogenation of one of three alcohols.
    % \item This allows us to also assess the capability of FineTuna to assess the trajectory of adsorbed slabs containing radicals. These molecules contain unpaired electrons and by nature are very unstable. As such, they are often prone to desorbing/dissociating which is not what we want(cite). If FineTuna can handle radical chemistry, it'll be very useful for rapidly calculating reaction diagrams.
    % \item In this experiment, we also wanted to gauge the ability of FineTuna to predict the trajectory when using a different functional from that of OC20 (rPBE). Here we assessed the use of the Bayesian Error Estimation Functional with a van der Waals dispersion correction (BEEF-vdW). 
    % \item Also gauge performance for facets that are OOD, MMI=3.
    % \item Since OC20 did not have dispersion corrections, the effects of physisorption were ignored. For large molecules such as those with more than two carbon atoms, intermolecular forces are dominant with chemisorption playing a minimal role(cite). Without dispersion corrections, these larger molecules will tend to exhibit desorption. This experiment will allow us to demonstrate the utility of FineTuna not just with small simple molecules, but with larger molecules as well.
% \end{enumerate}


% \usepackage{glossaries}
% \newacronym{oc20}{OC20}{Open Catalyst Project 2020}
% \newacronym{ocp}{OCP}{Open Catalyst Project}
% \newacronym{dft}{DFT}{Density Functional Theory}
% \newacronym{bfgs}{BFGS}{Broyden-Fletcher-Goldfarb-Shanno}
% \newacronym{cg}{CG}{Conjugate Gradient}
% \newacronym{ml}{ML}{Machine Learning}
% \newacronym{mlp}{MLP}{Machine Learning Potential}
% \newacronym{gpmin}{GPMin}{Gaussian Process Minimizer}
% \newacronym{gp}{GP}{Gaussian Process}
% \newacronym{ase}{ASE}{the Atomistic Simulation Environment Python package}
% \newacronym{gnn}{GNN}{Graph Neural Network}
% \newacronym{pca}{PCA}{Principal Component Analysis}
% \newacronym{ewt}{EwT}{Energies within Threshold}
% \newacronym{vasp}{VASP}{the Vienna Ab initio Simulation Package}
% \newacronym{mae}{MAE}{Mean Absolute Error}
% \newacronym{scf}{SCF}{Self-Consistent Field}
% \newacronym{rbf}{RBF}{Radial Basis Function}
% \newacronym{cbf}{CBF}{Circular Basis Function}
% \newacronym{sbf}{SBF}{Spherical Basis Function}
% \newacronym{pbe}{PBE}{Perdew-Burke-Ernzerhof}
% \newacronym{rpbe}{rPBE}{revised PBE}
% \newacronym{vdw}{vdW}{van der Waals}
% \newacronym{beefvdw}{BEEF-vdW}{Bayesian error estimation functional with van der Waals correlation}

% \ifthenelse{\boolean{anon}}{
%     \newacronym{vpi}{VASP interactive}{}
% }
% {
%     \newacronym{vpi}{VASPInteractive}{}
% }

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
